Geometrical Optics Formalism to Model Contrast in Dark-Field X-ray Microscopy

Dark-field X-ray microscopy is a new full-field imaging technique that nondestructively maps the structure and local strain inside deeply embedded crystalline elements in three dimensions. Placing an objective lens in the diffracted beam generates a magnified projection image of a local volume. We provide a general formalism based on geometrical optics for the diffraction imaging, valid for any crystallographic space group. This allows simulation of diffraction images based on micro-mechanical models. We present example simulations with the formalism, demonstrating how it may be used to design new experiments or interpret existing ones. In particular, we show how modifications to the experimental design may tailor the reciprocal-space resolution function to map specific components of the deformation gradient tensor. The formalism supports multi-length scale experiments, as it enables DFXM to be interfaced with 3DXRD. The formalism is demonstrated by comparison to experimental images of the strain field around a straight dislocation.

==> output.tex <==
%\input{output.bbl}

\referencelist[references]
